Wait-Free Updates and Range Search using Uruv

CRUD operations, along with range queries make a highly useful abstract data type (ADT), employed by many dynamic analytics tasks. Despite its wide applications, to our knowledge, no fully wait-free data structure is known to support this ADT. In this paper, we introduce Uruv, a proactive linearizable and practical wait-free concurrent data structure that implements the ADT mentioned above. Structurally, Uruv installs a balanced search index on the nodes of a linked list. Uruv is the first wait-free and proactive solution for concurrent B+tree. Experiments show that Uruv significantly outperforms previously proposed lock-free B+trees for dictionary operations and a recently proposed lock-free method to implement the ADT mentioned above.

==> algorithm/linked_list/WFinsert_ll.tex <==
\begin{algorithm}[H]
\label{WFllinsert}
\caption{\texttt{wfLLInsert}(key, value, tid, phase)}
\While{\textup{\texttt{true}}}
{
    llNode* $prevNode :=$ \texttt{nullptr}\;
    llNode* $nextNode :=$ \texttt{llFind}($key,\  \&prevNode$)\;
    \If{$nextNode ==$ \textup{\texttt{nullptr}}}
    {
        \textbf{return} \texttt{false}\;
    }
    \ElseIf{$nextNode \rightarrow key == key$}
    {
        \While{\textup{\texttt{true}}}
        {
            $currState := stateArray[tid]$\;
            \label{alg25:line294}
            \textbf{if} $currState \rightarrow finished$ || $currState \rightarrow phase \neq phase$  \textbf{then return} \texttt{true} \;\label{alg25:line295}
            $newVnode := currState \rightarrow vNode$\;
            \label{alg25:line296}
            $nextVnode := newVnode \rightarrow nextv$\;
            \label{alg25:line297}
            $currVhead := nextNode \rightarrow vhead$\;
            \label{alg25:line298}
             \texttt{initTs}($currVhead)$\;
             \label{alg25:init}
             $currValue := currVhead \rightarrow value$\;
            \label{alg25:line303}
            
            \If{$currState \rightarrow vnode \rightarrow ts \neq$ -1}
            {
                \label{alg25:line300}
                $currState \rightarrow finished =$ \texttt{true}\;
                \textbf{return} \texttt{true}\;
                \label{alg25:line302}
            }
            \textbf{if} \texttt{isMarked}($currVhead$) \textbf{then} \textbf{return} \texttt{false} \;
            \If{\textup{\texttt{wfVCAS}}($nextNode,\ currValue,\ value,\ newVnode,\ \newline
            nextVnode,\ currVhead  $)}{
            \label{alg25:line304}
            $currState \rightarrow finished := true$\;
            \textbf{return} \texttt{true}
            }
        }
    }
    \Else
    {
        $currState := stateArray[tid]$\;
        \textbf{if} $currState \rightarrow finished$ \textbf{then return} \texttt{true} \;\label{alg25:line308}
        \If{$phase \neq currState \rightarrow phase\  \&\& \ currState \rightarrow vnode \rightarrow ts \neq$ -1}
            {
                \label{alg25:line309}
                $currState \rightarrow finished =$ \texttt{true}\;
                \textbf{return} \texttt{true}\;
            }
        llNode* $newNode :=$ \texttt{new llNode}($key,\ value,\ currState \rightarrow vnode$)\;
        $newNode \rightarrow next := nextNode$\;
        \If{$prevNode \rightarrow next$.\textup{\texttt{CAS}}($nextNode,\ newNode$)}{
        \label{alg25:line314}
            \texttt{initTs}$(newNode \rightarrow vhead)$\;
            \label{alg25:line312}
            $currState \rightarrow finished := true$
            \textbf{return} \texttt{true}\;
        }
        \textbf{else if} \texttt{isMarked}($prevNode \rightarrow next$) \textbf{then return} \texttt{false}\;
    }
}
\end{algorithm}

==> algorithm/linked_list/init_ts.tex <==
\begin{algorithm}[H]
\label{llinit_ts}
\caption{\texttt{initTs}(Vnode)}
\If{$Vnode \rightarrow ts =$ -1}
{
    $currTs :=$ \texttt{getCurrTs()}\;
    $Vnode \rightarrow ts$.\texttt{CAS}(-1, $currTs)$\;
    \label{alg22:line270}
}
\end{algorithm}

==> algorithm/linked_list/insert_ll.tex <==
\begin{algorithm}[H]
\label{llinsert}
\caption{\texttt{llInsert}(key, value)}
\While{\textup{\texttt{true}}}
{
    llNode* $prevNode :=$ \texttt{nullptr}\;
    llNode* $nextNode :=$ \texttt{llFind}($key,\  \&prevNode$)\;
    \label{alg21:line252}
    \If{$nextNode =$ \textup{\texttt{nullptr}}}
    {
        \textbf{return} \texttt{false}\;
    }
    \ElseIf{$nextNode \rightarrow key = key$}
    {
        \While{\textup{\texttt{true}}}
        {
            $currVhead := nextNode \rightarrow vhead$\;
            \textbf{if} \texttt{isMarked}($currVhead$) \textbf{then} \textbf{return} \texttt{false} \;
            $currValue :=$ \texttt{read}($currVhead)$\;
            \textbf{if}\texttt{vCAS}($nextNode,\ currValue,\ value,\ currVhead $) \textbf{then} \textbf{return} \texttt{true}\;
            \label{alg21:line260}
        }
    }
    \Else
    {
        llNode* $newNode :=$ \texttt{new llNode}($key,\ value$)\;
        $newNode \rightarrow next := nextNode$\;
        \If{$prevNode \rightarrow next$.\textup{\texttt{CAS}}($nextNode,\ newNode$)}{
            \label{alg21:line264}
            \texttt{initTs}$(newNode \rightarrow vhead)$\;
            \label{alg21:line265}
            \textbf{return} \texttt{true}\;
        }
        \textbf{else if} \texttt{isMarked}($prevNode \rightarrow next$) \textbf{then return} \texttt{false}\;
    }
}
\end{algorithm}

==> algorithm/linked_list/read.tex <==
\begin{algorithm}[H]
\label{llread}
\caption{\texttt{read}(llNode)}
$currVhead := llNode \rightarrow vhead$\;
\texttt{initTs}$(currVhead)$\;
\label{alg23:line272}
\textbf{return} $currVhead \rightarrow value$\;
\end{algorithm}


==> algorithm/linked_list/vCAS.tex <==
\begin{algorithm}[H]
\label{llvcas}
\caption{\texttt{vCAS}(currNode, oldValue, value)}
$currVhead :=$ \texttt{unmarkedRef}$(currNode \rightarrow vhead)$\;
\texttt{initTs}$(currVhead)$\; 
\label{alg24:line275}
\textbf{if} $currVhead \rightarrow value \neq oldValue$ \textbf{then return} \texttt{false}\;
\textbf{if} $currVhead \rightarrow value = newValue$ \textbf{then return} \texttt{true}\;
Vnode* $newVnode :=$ \texttt{new Vnode}$(value)$\;
$newVnode \rightarrow nextv := currVhead$\;
\If{$currNode \rightarrow vhead$.\texttt{CAS}$(currVhead,\ newVnode)$}
{
    \label{alg24:line280}
    \texttt{initTs}$(newVnode)$\; \label{alg24:line281}
    \textbf{return} \texttt{true}\;
}
\textbf{else return} \texttt{false}\;
\end{algorithm}

==> algorithm/linked_list/wfVCAS.tex <==
\begin{algorithm}[H]
\label{wfllvcas}
\caption{\texttt{wfVCAS}(currNode, oldValue, value, newVnode, nextVnode, currVhead )}
\textbf{if} $currVhead \rightarrow value \neq oldValue$ \textbf{then return} \texttt{false}\;
\textbf{if} $currVhead \rightarrow value = newValue$ \textbf{then return} \texttt{true}\;
\textbf{if}$\, !\, (newVnode \rightarrow nextv.$\texttt{CAS}$(nextVnode, currVhead))$ \textbf{then return} \texttt{false}\;
\label{alg26:line320}
\If{$currNode \rightarrow vhead$.\textup{\texttt{CAS}}$(currVhead,\ newVnode)$}
{
    \label{alg26:line321}
    \texttt{initTs}$(newVnode)$\;
     \label{alg26:line319}
    \textbf{return} \texttt{true}\;
}
\textbf{else return} \texttt{false}\;
\end{algorithm}

==> algorithm/merge_helper.tex <==
\begin{algorithm}[H]
\label{mergehelper}
\caption{\texttt{mergeHelper}(rightChild,\ rightIdx,\ leftChild,\ leftIdx,\ prev,\ pidx,\ curr)}
\textup{Node*} $newNode$\;
\If{$rightChild \rightarrow count + leftChild \rightarrow count < MAX$}
{
    \textup{Node*} $newChild$\;
    \If{$leftChild \rightarrow isLeaf$}
    {
        $newChild :=$ \texttt{new LeafNode()}\;
        $newChild \rightarrow next := rightChild \rightarrow next$\;
    }
    \Else
    {
        $newChild :=$ \texttt{new InternalNode()}\;
    }
    Merge $rightChild$ and $leftChild$ into $newChild$\;
    \label{alg15:line185}
    \If{\textup{!}$\,leftChild \rightarrow newNext$.\texttt{\textup{CAS}}(\texttt{\textup{nullptr}}, $newChild$)}
    {
        \label{alg15:line186}
        $newChild := leftChild \rightarrow newNext$\;
    }
    $newNode :=$ \texttt{new InternalNode()}\;
    Copy every element in $curr$ into $newNode$ replacing pointers $leftChild$ and $rightChild$ with $newChild$\;
    \label{alg15:line189}
}
\textbf{else} $newNode :=$ \texttt{borrowHelper}($rightChild,\ rightIdx,\ leftChild,\ leftIdx,\ curr$)\;
\If{$prev =$ \texttt{\textup{nullptr}}}
{
    \If{$newNode \rightarrow count = 0$} 
    {
        $newNode := newChild$ \tcp*{this occurs only when the left and right children are merged and newNode has only one child}
    }
    \textbf{if} \textup{!}$\,root$.\textup{\texttt{CAS}}($curr, newNode$) \textbf{then} \textbf{return} \textup{\texttt{nullptr}}\;
    \label{alg15:line194}
}
\textbf{else if} \textup{!}$\,prev \rightarrow ptr[pidx]$.\texttt{CAS}($curr, newNode$) \textbf{then} \textbf{return} \textup{\texttt{nullptr}}\;
\label{alg15:line195}
\textbf{return} $newNode$\;
\end{algorithm}


==> algorithm/range_query.tex <==
\begin{algorithm}[H]
\label{range_query}
\caption{\texttt{rangeQuery}(low, high)}
vector<pair<key,value$>>$ $res$\;
int $ts :=$ \texttt{addTimestamp()}\;
\label{alg4:line83}
Node* $currNode := root$\;
\While{\textup{!}$\,currNode \rightarrow isLeaf$}
{
    Search $currNode$ for the appropriate child based on $key$\;
    Set $currNode$ to said child\;
}
Node* $prevNode :=$ \texttt{nullptr}\;
\While{$currNode \neq$ \textup{\texttt{nullptr}}}
{
\If{$currNode \rightarrow newNext \neq$ \textup{\texttt{nullptr}} $\&\& \ currNode \rightarrow newNext \rightarrow ts \leq ts$}
    {
        \label{alg5:line93}
        $currNode := currNode \rightarrow newNext$\;
        \label{alg5:line94}
        \textbf{if} $prevNode \neq$ \texttt{nullptr} \textbf{then} $prevNode \rightarrow next := currNode$\;
    }
    \Else
    {
        $res := list$.\texttt{rangeQuery}($low,\ high,\ ts,\ res$)\;
        $prevNode := currNode$,\ $currNode := currNode \rightarrow next$\;
        \textbf{if} $currNode \rightarrow list$'s first key $> high$ \textbf{then} \textbf{return} $res$\;
    }
}
\textbf{return} $res$\;
\end{algorithm}

==> algorithm/search_tree.tex <==
\begin{algorithm}[H]
\label{searchtree}
\caption{\texttt{search}(key)}
Node* $currNode := root$\;
\While{\textup{!}$\,currNode \rightarrow isLeaf$}
{
    Search $currNode$ for the appropriate child based on $key$\;
    Set $currNode$ to said child\;
}
llNode* $foundNode := currNode \rightarrow list$.\texttt{llFind}($key$)\;
\If{$foundNode \rightarrow key = key$}
{
    \textbf{return} \texttt{read} $(foundNode)$\;
}
\Else
{
    \textbf{return} -1\;
}
\end{algorithm}

==> algorithm/split_internal.tex <==
\begin{figure}[H]

% \renewcommand{\figurename}{Algorithm}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\begin{multicols}{2}

\end{multicols}
\end{figure}

==> algorithm/split_leaf.tex <==
\begin{algorithm}[H]
\label{splitleaf}
\caption{\texttt{splitLeaf}(prevNode,\ prevIdx,\ currNode,\ currIdx)}
$\textup{Node* } leftChild :=$ \texttt{new leafNode()}\;
$\textup{Node* } rightChild :=$ \texttt{new leafNode()}\;
$leftChild \rightarrow next := rightChild$ \; \label{alg19:line237}
$rightChild \rightarrow next := next$ \;
Split \textit{\textbf{this}} node into a pair of nodes pointed to by $leftChild$ and $rightChild$\;
\label{alg19:line233}
\If{\textup{!}$\ newNext$.\texttt{\textup{CAS}}($nullptr,\ leftChild$)}{
    \label{alg19:line234}
    $leftChild := newNext$\;
    $rightChild := leftChild \rightarrow next$\;
}

$\textup{Node* } newNode :=$ \texttt{new internalNode()}\;
Copy elements from $currNode$ to $newNode$ replacing $currChild$ with the two pointers $leftChild$ and $rightChild$\; \label{alg19:line239}
\If{$prevNode =$ \textup{\texttt{nullptr}}}
{
    \textbf{if} \textup{!}$\,root$.\texttt{CAS}($currNode,\ newNode$) \textbf{then} \textbf{return} \texttt{nullptr}\; \label{alg19:line241}
}
\textbf{else if} (!$\,prevNode \rightarrow ptr[prevIdx]$.\texttt{CAS}($currNode,\ newNode$) \textbf{then} \textbf{return} \texttt{nullptr}\; \label{alg19:line242}
\textbf{return} $newNode$\;
\end{algorithm}

==> algorithm/version_tracker/add_timestamp.tex <==
\begin{algorithm}[H]
\label{addtimestamp}
\caption{\texttt{addTimestamp}()}
\While{\textup{\texttt{true}}}{
    $currTail := tail$\;
    TrackerNode* $\ newTail :=$ \texttt{new TrackerNode}$(currTail \rightarrow ts + 1 ,\ sentinelLast)$\;
    \If{$currTail \rightarrow next$.\textup{\texttt{CAS}} $(sentinelLast,\ newTail)$}{
        $tail$.\texttt{CAS}$(currTail,\ newTail)$\;
        \textbf{return} $newTail \rightarrow ts$\;
    }
    \Else{
        \While{\textup{\texttt{true}}}{
            $currTail := tail$\;
            \textbf{if} $currTail \rightarrow next = sentinelLast$ \textbf{then return}\;
            \textbf{else} $tail$.\texttt{CAS}$(currTail,\ currTail \rightarrow next)$\;
        }
    }
}
\end{algorithm}

==> algorithm/version_tracker/get_latest_timestamp.tex <==
\begin{algorithm}[H]
\label{getlatestts}
\caption{int \texttt{getLatestTs}()}
\textbf{return} $tail \rightarrow ts$\;
\end{algorithm}

==> sections/LP.tex <==
As explained earlier, we traverse down Uruv to the correct leaf node and perform all operations on the linked-list in that leaf. Therefore, we discuss the LPs of the versioned linked-list.
\vspace{-0.2cm}\paragraph*{Insert.} There are two cases. If the key does not exist, we insert the key into the linked-list at line \ref{alg21:line264} or \ref{alg25:line314}. However, the key’s versioned timestamp is invalid, and it can only be made valid using \texttt{initTs} after the first successful execution of line \ref{alg22:line270}. This can be executed either by insert at line \ref{alg21:line265} or \ref{alg25:line312}, some concurrent read at line \ref{alg23:line272}, or some concurrent update at line \ref{alg24:line275} or \ref{alg25:init}.

If the key already exists, we update its value by atomically replacing its current $vhead$ with a new versioned node inside \texttt{vCAS} at line \ref{alg24:line280} or inside \texttt{wfVCAS} at line \ref{alg26:line321}. After successfully changing the $vhead$, the node’s timestamp is still invalid, and it can only be made valid using \texttt{initTs} after the first successful execution of line \ref{alg22:line270}. This can be executed either by \texttt{vCAS} at line \ref{alg24:line281} or by \texttt{wfVCAS} at line \ref{alg26:line319}, some concurrent read at line \ref{alg23:line272}, or some concurrent update at line \ref{alg24:line275} or  \ref{alg25:init}.

Line \ref{alg22:line270} is the LP for insert. Whenever we read any key’s value from its versioned node, we need to make sure the versioned node’s timestamp is valid. This ensures that a range query fetches all the relevant keys and their values present when the range query was invoked. Otherwise, if the LP is given to some line earlier than \ref{alg22:line270}, the key could have existed, but a concurrent range query can miss it, leading to inconsistency. 
\vspace{-0.3cm}\paragraph*{Delete.} There are two cases. If the key does not exist, then there is no need to delete the key as it does not exist. Therefore, the LP would be line \ref{alg20:line243}, where we last read a node from the linked-list. Instead, if the key exists, since we perform an update at line \ref{alg9:line132} or \ref{alg10:line151}, the LP would be the same as insert’s, which is line \ref{alg22:line270}.
\vspace{-0.2cm}\paragraph*{Search.} Regardless of whether the key exists or not, search's LP would be line \ref{alg20:line243} when we first read the node whose key is greater than the key we are searching for in the linked-list. If a concurrent insert/delete leads to a split/merge operation, then there is a chance that search will end up at a leaf node that is no longer a part of Uruv. In that case, search’s LP would have happened before insert/delete’s LP. Search’s LP remains the same as above.
\vspace{-0.2cm}\paragraph*{Range Query.} In a range query, we call the \texttt{addTimestamp} method, which updates the global timestamp and returns that. So the LP for range query would be the successful execution of line \ref{alg4:line83}. The range query’s LP will remain the same regardless of any other concurrent operation.


==> sections/introduction-old.tex <==
Concurrent data structures have become very important due to their significant performance benefits over sequential data structures in multicore environments. Active research continues in this area resulting in new sophisticated and efficient concurrent data structures every year. Naive concurrency tends to use mutexes. When multiple threads need to update a data structure, access is granted to only one thread at a time. This technique ensures updates do not get corrupted. However, there is a drawback. Since mutexes enable mutual exclusion, a thread, $t_1$, has to potentially wait for another thread, $t_2$, to finish its operation before accessing the data structure. If thread $t_2$ crashes or slows down considerably, thread $t_1$ will end up waiting indefinitely or for a long time. This will affect the data structure’s performance.

Another type of concurrency called non-blocking concurrency can potentially mitigate the drawback. In this approach, concurrency is achieved without using mutexes. Atomic operations like \texttt{compare-and-swap (CAS)} are used to achieve necessary modifications in the data structure. We deal with lock-free and wait-free non-blocking concurrency. A significant attraction of lock-free concurrency is its progress guarantee: \textit{If multiple threads perform operations on a lock-free data structure, at least one of them will complete its operation given enough time.} A much stronger progress guarantee is provided by wait-free concurrency, wherein operations finish in a finite time.

Many lock-free data structures have been developed in recent years, including but not limited to linked lists, BSTs and queues. However, not much work is done for a lock-free B$^+$Tree. According to our literature review, Anastasia et al.\cite{braginsky+} proposed the first and only lock-free B$^+$Tree. Their tree uses a data structure, chunk, that can perform concurrent insert, delete and search operations on their nodes. Chunk is a continuous memory block where these operations can be performed with the help of a  lock-free linked list. We have developed an efficient lock-free ranged tree data structure, called Uruv, that is inspired by the B$^+$Tree’s design. Updates to Uruv are lock-free, and lookups and range queries are wait-free.

The state of a data structure is defined by the keys and the data it contains. Sometimes, a subset of keys within some given range and their data is required. Range queries are operations that return a set of all the keys and their data in a data structure within a given range. The B$^+$Tree is a ranged index that inherently supports ranged queries. Making a range query concurrent with other operations is essential for data structure performance in a multi-threaded environment. A naive way to perform a range query is by locking a part of the data structure that belongs to the range. This faces the same performance problems we discussed regarding lock-based data structures. A lock-free range query achieves this result without using mutexes, enabling lock-free performance guarantees. We build on the work of Wei et al.\cite{wei2021constant}, who propose a constant-time lock-free snapshot algorithm. Their algorithm works by storing multiple versions of keys in a data structure. Each key’s version is identified by timestamp and stores data the key was mapped to at that time. (TO-DO Add related work for range query)

We begin by summarizing the B$^+$Tree's design in Section \ref{sec:Preliminaries}. We then explain Uruv's design in Section \ref{sec:Design}. We detail important algorithms in Section \ref{sec:main_algo} and have detailed other algorithmic details in the Appendix. (TO-DO Update this paragraph once every later section is completed)

==> sections/rebuttal.tex <==
We sincerely thank the reviewers for taking the time to review our submission. In the following, we address their questions and concerns.

Response to Reviewer 1:

a) Presentation-wise, the paper is not self contained. ... pseudo-code and its description to Appendix.

Response: We appreciate this suggestion. We are hopeful that the reviewer would agree with our observation that writing the description of an “advanced” non-blocking data structure in a conference paper has been getting trickier over the last few years with the growing complexity of such works. These data structure algorithms invariably consist of many non-trivial details. Some readers/reviewers prefer a high-level overview first and yet others say that details were missing. As an author, it becomes hard to opt for a style. We will try our best to restructure the paper in the final version.

b) Related to the above, the trickiest part of any concurrent balanced tree algorithm is rebalancing. This paper does not provide enough details to convince me that it “solves” this problem correctly. 

Response: A node is balanced by freezing the current node and its parent when rebalance needs to be triggered. Then a new node, or, two new nodes, are created to replace the current node, depending on the case for a merge or a split. While a node is frozen, helping is performed by threads that access it. These are described in the paragraphs “Freezing/Marking”, “Balancing a Leaf”, “Split”, and “Merge” in Section 3. The relevant lines of the algorithm are described therein.


c) In particular, based on the code in Algorithm 1 (that is included in the paper) it is unclear what happens if a thread reads keys in a node while that node is being concurrently replaced through merged/split. 

Response: The read operations have an oblivious traversal. They pass through a frozen node and have a linearization point before that of the update operation which either triggered helping or got into helping for rebalancing as described above. 

d) Couldn’t that Insert end up in a “wrong” leaf?  

Response: Update operations (insert/delete) perform “proactive traversal” as described in paragraphs “Insert into Uruv” and “Deleting from Uruv” and the relevant lines referred to therein. It essentially means that an insert operation helps a frozen internal node as well.

e) Also, given that read operations (find and range query) do not engage in rebalancing, it seems like logarithmic complexity of those operations might be compromised (as the tree might be completely out of balance due to numerous updates).

Response: As described, the proactive traversal by updates ensures that the tree is not too off-balance. The complexity incorporates the interval contention $I_C$ as described in Section 5.4.

f) Design-wise, the paper should discuss the memory management issue. ... need to be addressed carefully. 

Response: We physically delink the deleted nodes when they are “out of requirement” by range queries going by the version numbers while performing split or merge operations. We believe it is fairly standard to outsource the memory reclamation task to existing memory management methods.

g) Performance-wise, there are two separate issues. First, the paper should explain better the achieved results. What is the LFB+ tree (citation?) and why is it 95x slower in read-only workload? Intuitively, there is absolutely no reason for a lock-free B+-tree to be slower than Uruv when no range queries are concerned, certainly not by almost two orders of magnitude. 

Response: LFB+ Tree (cited as [4], unfortunately, we missed it in Section 6; however, we have mentioned that in point (e) in the last paragraph of Section 1 and elsewhere as well) is indeed an “interesting” implementation, which we too wondered why it performs so poorly when we saw that for the first time. To begin with, we have taken the author’s implementation. We could not find any work that evaluated this implementation after it was published. In their paper, they compared it against their own lock-based implementation. More technically, it uses the contiguous memory chunks to store a linked list in a manner that its nodes will be stored in some (not necessarily exactly contiguous location) cell of an array. This is the way they implement both internal and leaf nodes. At every level, they do a linear search in such linked lists. Thus they roughly pay $O(B log_B n)$ for a search instead of $O(log_2 B log_B n)$, which Uruv and other standard B-trees do by doing a binary search at every level (Uruv does linear at leaf levels). This arrangement at the leaf node not only does not help in any manner whatsoever but also makes it too costly to allocate new nodes. We were indeed surprised to see a performance of loss of two orders of magnitude by this. We decided not to include this analysis in the submission, however, it is reasonable that a reader will be intrigued by these numbers. We are now planning to drop this data structure in the final version instead of including it.

h) A similar question applies to the comparison with VCAS-BST -- why is Uruv better, especially when the workload has more reads (see Figure 6)? Wait-freedom alone cannot explain this difference since the tree is huge and the operations should hardly get any help to complete (though including some stats about restarts would be helpful).

Response: Uruv being a B+-tree has smaller height compared to unbalanced BST. The suggestion about stats is a good suggestion -- we will try including it in the final version.

g) Second, there are several baselines... they should be included in the evaluation.

Response: We have the comparative numbers of [5] and [7]. Uruv does better than C-IST [7] in many settings, however, AB-tree [5] always outperforms Uruv. We essentially compared Uruv against “only B+-trees”. Nevertheless, we shall include those numbers too in the final version. Nelson et. al. [18] is lock-based and therefore we did not include that in the comparison. That work will be better compared to VCASBST. Thank you for pointing to Bz-tree; we compared against Bw-tree [21] and now know that Bz-tree outperforms it in several settings. We will include that too in the final version. 



We thank the reviewer for each of the minor comments, which we will definitely address along with a more thorough proofread.

Response to Reviewer 2:

a) The novel aspects of the design and the analysis could be better highlighted since this would clarify the significance of your contribution. It appears that most of the construction uses prior results from references [11,22] in the lock-free design, and then from [20] to achieve a wait-free version.

Response: We have several non-trivial constructions, beyond drawing from the existing ones mentioned by the reviewer. For example, wfVCAS required maintaining the version updates in the state-array indices corresponding to the operations, starting from the very allocation of a node, which the existing vCAS did not have to face, nor the wait-free non-versioned data structures. Similarly, the proactive traversal by concurrent updates is highly effective for our purpose which we believe was not explored by the related work. We thankfully accept this remark, we will highlight this in the final version.  

b) The arguments for correctness seems somewhat informal. It might benefit the presentation to have a lemma/theorem format, along with proofs, even if those need to be pushed to an appendix or online version. I found the absence of technical arguments a little strange.

Response: We accept that the correctness arguments are in form of “proof sketches”. However, they are not too away from the standard; for example, see C-IST [7]. We plan to write the correctness arguments in a formal way in an extended/journal version of this paper.

c) Sometimes this isn’t... that much worse.

Response: We have addressed this in Response to Reviewer 1. The error bars are not significant. Number of trials as 7 is fairly standard in the literature.

Response to Reviewer 3:

a) In particular, the paper sells Uruv ... “trick” or “insight” that Uruv makes use of in its design.

Response: We thank the reviewer for this remark. We will restructure the paper in the final version to highlight our contribution.

b) Furthermore, the algorithm ... As such, I found it difficult to verify correctness.

Response: We have a high-level description in form of Figure 3. Furthermore, in section 3 and 4 we give a high-level description of lock-free/wait-free insert/delete before actually delving into those. Beyond this it was difficult to include another section/subsection on “High-level Description” under the space budget. We however acknowledge your remark and will restructure to bring the short descriptions of insert/delete operations from Sections 3 and 4 to a dedicated section for quick reference to a reader.

c) In the early description of the protocol in section 3, ... the total number of nodes (i.e. deletions don’t shrink the tree)?

Response: We have addressed a similar concern in point (f) of Reviewer 1 above.

d) While the experimental results are impressive, they are not explained at all. What about Uruv’s design.... What happens in long runs when the lack of garbage collection starts being problematic?

Response: We have already explained above in point (g) to Reviewer 1 the issues with LFB+ tree [4]. Uruv actually uses a wait-free variant of vCAS as explained above. Your observation is correct to an extent that the range-queries become “comparatively” slower with an increase in their percentage in Uruv. This is expected because with (reasonably high) updates many leaf nodes could be under split. Range search in Uruv “links” those nodes at leaf level wherever encountered. In vCASBST, they do not face this issue. However, in absolute numbers, Uruv still does better. For sure, if there are only range searches without updates, Uruv will outperform BST because of its smaller height. Essentially, we may expect some spots on the horizon of workloads, where vCASBST will outperform Uruv, however, that will be too occasional.


e) Figure 6d is not described properly; the distribution of operations does not add up to $100\%.$

Response: This was a typo mistake. Thanks for pointing it out.

f) Other comments and suggestions.

Response: Thank you very much for your remarks on the proofread. We will thoroughly work on that in the final version.
